LLM-Evaluation Tropes: Perspectives on the Validity of LLM-Evaluations

Large Language Models (LLMs) are increasingly used to evaluate information retrieval (IR) systems, generating relevance judgments traditionally made by human assessors. Recent empirical studies suggest that LLM-based evaluations often align with human judgments, leading some to suggest that human judges may no longer be necessary, while others highlight concerns about judgment reliability, validity, and long-term impact. As IR systems begin incorporating LLM-generated signals, evaluation outcomes risk becoming self-reinforcing, potentially leading to misleading conclusions. This paper examines scenarios where LLM-evaluators may falsely indicate success, particularly when LLM-based judgments influence both system development and evaluation. We highlight key risks, including bias reinforcement, reproducibility challenges, and inconsistencies in assessment methodologies. To address these concerns, we propose tests to quantify adverse effects, guardrails, and a collaborative framework for constructing reusable test collections that integrate LLM judgments responsibly. By providing perspectives from academia and industry, this work aims to establish best practices for the principled use of LLMs in IR evaluation.

==> guardrails-snifftests.tex <==

\section{Guardrails and Sniff-tests \ld{needs better name}}
\ld{I assume we at some point want to stop studying LLM-evaluators against manual data, and want to reap the fruits of our labor and write some systems papers with them.}

\ld{Under which conditions do we think this is a valid paradigm?}

\ld{What sniff-tests to we want to conduct or guardrails to put in place for us to trust a research paper written with LLM-evaluation?}

\ld{What are limits or constraints, where we would need to stop and do more examination?}


\section{Nick's thoughts on multiple complementary metrics}
Charlie’s “then you are done” statements are specifically what I’m truing to exclude, i.e. circular eval. Need to (a) evaluate a “shippable umbrela” vs humans, or (b) eval your shippable system using multiple diverse approaches: {\sc {\sc umbrela}}, laura rubrics and charlie llm-based pairwise eval. If those three llm eval methods are validated vs humans (i.e. each pretty good), and diverse, and positive on multiple tests, it’s harder to argue we overfitted to things that humans don’t care about. Let’s discuss adjusting the criteria if people see flaws, but the goal is to both improve the expensive unshippable models (a) and improve the system (b). Make it clear what those two types of paper look like.

his overfitting thing is not unique to llm metrics. The story I told at swirl about using multiple metrics was about Amit Singhal (happened at bing too), so maybe 10-20 years ago at google. It’s a guess on my part actually, from being in the industry a long time and observing things (e.g. talking to a disgruntled ML person about how Amit is anti-ML).
Some ML person would train the hell out of the system on some metric, e.g. their ndcg labels. ML person would say “I’m a genius, let me completely replace Amit’s ranker”. Amit would refuse to let that system take over, because although it had higher ndcg it has lower click+dwell (and other metrics regress too), and at some stage what’s the point of retrieving results with somewhat higher labels of users are significantly less likely to see (click) them. Could be cases where caption is bad so the user doesn’t know to click. Could be cases where ndcg judge misunderstands/misguesses the real user intent. Could just be things that ndcg labeling doesn’t try to catch (e.g. this user already read page A, the most relevant page, although the system has no record of this, so they will click page B today, but that’s not a reason to give A a lower label). The ranker should not ship, i.e. measurably worse on multiple metrics and maybe also harder to debug and maintain.
Similar thing if the genius wanted to do ml on clicks only, the new ranker would fail on ndcg and spam metrics, etc. Amit forced people to build a balanced system, rather than focus on one aspect only and try to declare victory. We had a very similar learning process in Bing, i know because i worked on it. So I’d say Laura your concern is correct, and exacerbated with llm metrics if they are more gamble, but this issue of overfocus on one metric has been an issue anytime you are using a bunch of surrogate metrics, none of which perfectly capture user experience. This is a key point to understand!!!
Part of what we may be doing here is translating these practices from industry to the SIGIR community. We already prefer to see multiple test collections in a sigir paper, maybe we are pointing out the importance of enforcing (an updated version of) that kind of anti-overfitting thing.

\ld{One issue that I see is that most of the trec\_eval metrics are highly correlating with one another}

Highly correlated: Yeah two concerns here. 1) Our metrics are not diverse enough (we have nothing that’s as different as ndcg vs clicks vs spam detector vs etc). 2) The diverse llm metrics we have, such as ndcg vs pairwise tournament vs sbs list-vs-list, have correlated weaknesses e.g. all susceptible to keyword stuffing.
Maybe the research community can solve problems 1+2 by actively developing the right suite of metrics.



\subsection{Privileged Information and a False Sense of Security}

A common argument in favor of nuggetized (or grading rubric) evaluation approaches is that since nuggets are manually created, they represent privileged information---knowledge that no LLM could independently infer.  

However, this assumption warrants closer scrutiny. LLMs have demonstrated the ability to generate plausible nuggets for a given query, even without explicit context \ld{Cite pencils exam++}. Furthermore, if an LLM is provided with a few manually created nuggets as exemplars, it may generalize effectively, producing nugget-like responses that closely align with human-created rubrics.

\paragraph{Turing Test for Nugget Prediction}  
This raises an important question: Should nugget generation be subjected to a Turing test? If LLMs can reliably guess what a human would consider relevant---even without explicit exposure to the full grading rubric---then the assumption that manually defined nuggets serve as privileged information may not hold.  

A major risk of this scenario is the unintended introduction of an LLM Ranker that implicitly encodes privileged information. In such cases, a method developer may believe they are submitting a Traditional System (Dim 3) but, in reality, their system incorporates an LLM-judge reranker that optimizes for human-like relevance signals. This could distort evaluations, creating an illusion of generalization while merely replicating the evaluator’s biases.

\paragraph{Key Questions for Further Study}  
The following questions highlight open challenges in determining the validity of LLM-assisted evaluation:  
\begin{itemize}  
    \item Can only humans reliably judge relevance?  
    \item Are LLMs viable replacements for human assessors?  
    \item Are LLMs capable of perfectly predicting what a human judge would say?  
    \item If an LLM could match or exceed human judgments, should it be considered a better judge than an average human assessor?  
    \item How should a better LLM judge be defined? By its agreement with human annotations, its ability to generalize relevance, or its consistency across queries?  
\end{itemize}  

\bigskip

This issue also connects to concept drift: If multiple LLMs consistently agree that certain responses are relevant, but human users perceive a decline in search quality, it suggests that LLM evaluations may be drifting away from real user needs. Over time, reliance on LLM-generated assessments may reinforce a misaligned feedback loop, leading to gradual degradation in practical retrieval effectiveness.


% A common argument made in the context of nuggetized (or grading rubric) evaluation approaches is that because Nuggets are manually created, these represent privileged information that no LLM could know.

% % E.g. are LLMs capable of guessing which nuggets/questions a human would put on a grading rubric for a query?
% One concern with this reasoning is that LLMs have demonstrated that they can produce convincing nuggets on a given query. This has been demonstrated even  without providing context \ld{Cite pencils exam++}, but one could also imagine  providing with a few manually created nugget examples as exemplars.


% Maybe we should submit nuggets to a Turing test, to study whether LLM's can guess what is relevant anyway. If this is the case, then there is a high danger of an unintended consequence, where an LLM Ranker is incorporated into the system that guesses the privileged information. In this case a method developer may believe they submit a Traditional System (Dim 3), but actually the system includes an LLM-judge ranker.


% % Setting aside LLM-usage for cleanup and syntactic support tasks, and focusing on the core of what is relevant.

% The following questions deserve further study:
% \begin{itemize}
%     \item Are only humans able to judge the relevance?
%     \item Are LLMs good replacements for humans?
%     \item Are LLMs even better at determining relevance than humans? (Or are they 
%     able to perfectly guess what a human would say)
%     \item Would a perfect LLM judge be better than human or the ``average human'' 
%     assessor? 
%     \item How do we define a better LLM judge?
% \end{itemize}




% \ld{..} This links to the issue of Concept drift: multiple LLMs agree that something is relevant, but the human wonders why the search results are getting worse and worse





\subsection{LLM-Human Coworking in Judgments}
\label{sec:llm-human-coworking}

A commonly debated approach in evaluation is one where an LLM-judge produces initial relevance labels, which are then verified by a human judge (links to 4.1). This hybrid method aims to combine the scalability and consistency of LLMs with the nuanced reasoning of human assessors. However, significant challenges arise in this collaboration, particularly regarding overreliance on LLM outputs.

\paragraph{The Issue of Overreliance}  
Humans exhibit a well-documented cognitive bias toward deferring to machine-generated outputs, even when such reliance is unwarranted \ld{cite fork \& weld}. In the context of LLM-assisted evaluation, this can lead to blind faith in LLM-generated judgments, causing assessors to accept system-proposed labels without sufficient scrutiny.  

One consequence of this bias is that the same human annotator may produce different judgments depending on whether they see the LLM’s proposal first. This suggests that LLM-provided labels may subconsciously anchor human decisions, affecting evaluation reliability.  

\paragraph{Vigilance Testing for Overreliance}  
A core practice in security agencies such as the TSA is to conduct vigilance tests---periodic interventions designed to keep human checkers alert and engaged. Inspired by this approach, we propose using vigilance testing as a diagnostic tool to measure the extent of human overreliance on LLM-generated labels.

For binary relevance labels, a random subset of cases could be subjected to inverted LLM proposals---where the LLM's original label is flipped. If assessors fail to correct the inverted label, this indicates an implicit bias toward agreeing with the LLM’s suggestion rather than independently verifying the judgment.

By comparing the agreement rate on standard vs.\ inverted LLM proposals, we can quantify the extent to which human annotators are over-relying on the LLM output. This test could be further extended by informing annotators post-hoc that the label was inverted and asking them to provide a rationale for their final decision, offering deeper insights into whether overreliance is driven by cognitive bias or trust in model accuracy.

\paragraph{Future Research Directions}  
Understanding human overreliance on LLM outputs is crucial for designing hybrid evaluation frameworks that preserve human critical judgment while leveraging LLM efficiency. Future work should explore:
\begin{itemize}  
    \item How the order of presentation (LLM-first vs.\ human-first labeling) affects judgment.  
    \item Whether annotators consciously recognize their tendency to agree with LLM proposals.  
    \item If certain types of queries or labels are more susceptible to overreliance effects.  
\end{itemize}  
Addressing these questions will help establish guardrails that maintain evaluation integrity in human-LLM coworking setups.


% \ld{This is a particular challenge that could also fall under the "guardrails" category}

% A commonly debated idea is one where an LLM-judge produces labels which are verified by a human judge.


% \paragraph{Issue of Overreliance.}
% However, due to a cognitive bias humans tend to overrely on a the LLM output \ld{cite fork \& weld}, leading to blind faith in the LLM judgment even when not warranted. This may result in the phenomenon where the same annotator would arrive at a different label when shown the LLM proposal than by themselves.

% \paragraph{Vigilance test.}
% A core practice at security agencies  such as the TSA, is to regularly conduct Vigilance tests, to ``keep the human checkers on their toes''.
% We use this idea to devise a test to measure the amount of overreliance-bias in humans as follows.

% For binary relevance labels, in a random percentage of cases, we invert the proposal of the LLM-evaluator, so that in order to agree with the LLM-evaluator, the human would need to change the (inverted) LLM-label. If the human fails to change the label, we count this as a disagreement with the (original) LLM-judge proposal.

% We can compare the population of agreements on both the inverted and untreated LLM-proposals, to measure the human overreliance bias.

% The test could be extended by revealing to the human that the label was inverted, and asking for a rationale on their choice.



% \ld{I asked Rob Capra for some citations on the TSA test, below his response}

% \ld{..} Terms to search for are "vigilance task", "vigilance task performance", and "cognitive vigilance task".  It is a large area of study, so you probably want to find a citation that matches your scenario.  Here are a few to get you pointed in the right direction.

% \url{https://www.sciencedirect.com/topics/medicine-and-dentistry/vigilance-task}

% \url{https://sciences.ucf.edu/psychology/perl/wp-content/uploads/sites/29/2019/08/The-effects-of-event-rate-on-a-cognitive-vigilance-task..pdf}





% \subsection{Pro and con debate and judge}

% \ld{..} debate ideas 

% \subsection{Reasoning chain of thought}
% for both human and llm 
% Need to validate the evaluation, task on different steps, not just the final result.
% In process evaluation/validation. Defining some subjective criteria for the validation / evaluation 

\subsection{Pro-Con Debate and Third-Party Judgment}  
An alternative approach to guardrail LLM evaluations is to introduce a structured debate framework \ld{cite debate /kahn}, where two LLMs adopt opposing stances on a relevance judgment---one arguing for relevance and the other against. This adversarial setup ensures that the justification for relevance is explicitly articulated, rather than simply relying on an implicit scoring function.  

Once the debate is complete, a third-party judge---either an LLM or a human---evaluates which argument is more convincing. This approach could:  
\begin{itemize}  
    \item Surface edge cases where relevance is ambiguous.  
    \item Encourage explicit reasoning rather than opaque binary judgments.  
    \item Reduce bias amplification, as opposing viewpoints must be defended.  
\end{itemize}  

By forcing LLMs to explicitly justify their relevance assessments, this method may help identify inconsistencies in evaluations and provide a richer explanation structure for relevance decisions.

\subsection{Reasoning Chains and Stepwise Validation}  
Another potential guardrail approach is to shift from single-step evaluations toward stepwise reasoning validation---a method that applies to both human and LLM-based evaluations. Instead of judging only the final output, intermediate decision steps should be evaluated and validated.  

This aligns with ideas from reasoning chains, such as the multi-step reasoning observed in GPT o1 and o3 models. In such models, explicit reasoning chains improve transparency and robustness. Similarly, requiring humans and LLMs to articulate their reasoning at multiple steps would allow:  
\begin{itemize}  
    \item Validation of intermediate steps, ensuring logical consistency.  
    \item Identification of subjective criteria that influence final evaluations.  
    \item Detection of systematic biases that may emerge during multi-step judgments.  
\end{itemize}  

Rather than treating relevance assessment as a black-box classification task, incorporating stepwise reasoning could make evaluations more interpretable, auditable, and reliable.





==> long-opinions.tex <==
\section{Perspectives of Co-Authors}
\label{sec:perspectives}

\begin{description}
    \item[\Charlie{}: ] I believe LLMs can be effectively (not necessarily
          efficiently) used as re-rankers, particularly with {\sc Umbrela}, to
          achieve near-perfect results for traditional relevance if LLMs are
          accepted as judges. However, I acknowledge the potential cost of using
          {\sc Umbrela} as a final-stage ranker. Beyond traditional relevance, I
          am interested (similarly to \Nick{}) in using LLMs (or no LLMs?) to
          interpret/investigate implicit feedback like click data to understand
          user information needs better and investigate the discrepancies
          between implicit feedback metrics and human relevance labels. I see
          potential in LLMs to advance beyond the Cranfield paradigm but
          disagree with the idea that {\sc Umbrela} (or any other single LLM
          judge) is a singular solution for all ranking needs.
          % He argues that (a) is crucial for establishing trust, enabling (b),
          % but warns against circular validation (the evaluator is also the
          % ranker) and advocates for more focus on building deployable systems,
          % especially as the line between (a) and (b) blurs with decreasing
          % computational costs. This can potentially be achieved with LLMs used
          % for evaluation beyond just topical relevance judgments but while
          % ensuring alignment with human users/assessors throughout the
          % process.


    \item[\Faegheh{}:] LLM-based evaluations are essential to develop future
          Information Access that are beyond current SERP. The search space is
          complex and the involvement of humans during optimization is not
          practical. We need to have a reliable automatic evaluation to optimize
          the method. Once we land on a local optima, human evaluation can find
          the problems, and the models can be further developed and optimized.


    \item[\Peter{}:] LLMs provide a mechanism to introduce human-like
          variability into test collection evaluation at a scale and in
          controlled ways that are not realistically possible to perform with
          actual humans. But the end purpose is for humans to use the systems
          that get built subsequently, so they have to be introduced at some
          point to validate outcomes. Interleaving is a high efficiency
          framework to conduct that with people, if A/B testing is prohibitive.


    \item[\Ellese{}:] I believe the usefulness of LLM evaluators at replacing
          human relevance judgments has been demonstrated across various
          studies, as well as in our own experience. However, current models
          still have limitations and can exhibit unexpected behavior and issues
          with instruction following, so I think it is still important to have a
          level of human oversight to validate the output from LLM evaluators.
          This can be at a vastly reduced scale from the number of humans that
          would be required to manual generate these judgments, requiring only
          the input of a few human ``experts'' on a sample of data. In the
          future, I could see a time where this oversight is mostly or even
          completely replaced with AI methods, such as using a more powerful
          model in place of a human reviewer, and monitoring appropriate metrics
          rather than having manual human validation of data.



    \item[\Nick{}:] I want to distinguish between two types of IR research: (a)
          developing expensive models of human preferences and behavior,
          validated against real people, and (b) building practical, deployable
          systems, validated against a variety of human data and/or expensive
          (a) models. The community should encourage activities of type (a), to
          develop better metrics for search, RAG, conversation, personalization,
          citation, hallucination, etc. Models must be validated against real
          human data, repeatedly, and new papers that find flaws in the metrics
          (mismatch with human preferences) will make good SIGIR papers as
          always. Meanwhile, the community should also not forget to build IR
          systems that can be deployed. IR systems are foundational in our
          field, and as the richness of type (a) models rush ahead, there should
          be research of type (b) to reduce those expensive models to a
          ``shippable'' system. Since we have multiple forms of evaluation, and
          any one can be biased, the field should require multiple metrics in a
          paper of type (b). For example, improving both nugget recall and
          citation precision/recall, or improving both NDCG and clicks from a
          simulated user. This is similar to the previous requirement at SIGIR
          of using multiple test collections. The goal is to provide evidence of
          a real improvement---rather than accidental results due to overfitting
          towards a single metric/dataset.


    \item[\Laura{}:] I want to add to \Oleg{} that I don't find it easy to trust
          direct prompting approaches like {\sc umbrela}, mainly because I don't
          see a good way to incorporate humans without biasing them to agree
          with the LLM. I have more trust in a nuggetized approach or some other
          means of breaking down ``relevance'' into more specific components
          that can be individually checked. This would also combat the Blackbox
          Labeling trope.

          Another concern is the reliance on API-based LLMs, such as {\sc
          umbrela}, and its implications for the future of IR research. If the
          underlying model were to change significantly or become unavailable,
          it could render prior research results un-reproducible.


    \item[\Mark{}:] I don't think we can fire all humans, but I think it is
          important to recognize that there are different levels of human
          judgment quality. About 16 years ago we saw that we could use
          Crowdsource workers for relevance assessment and I think what we're
          finding with LLMs is that we can mostly replace those workers with an
          automated labeling approach. However, those labels need to be
          validated against high quality human relevance assessments.


    \item[\Oleg{}:]  We need an ongoing ``Coopetition'' framework for evaluating
          IR systems and LLMs as evaluators to instill trust. This would involve
          two types of submissions: systems tackling a specific task with
          various approaches and LLM evaluators judging these systems. The goal
          is to produce a test collection with human and top-performing
          LLM-evaluator labels, ideally with a publicly available implementation
          for broader use and to address judgment holes. We envision a yearly
          iteration of this process with new tasks, queries, and potentially
          updated ``best'' LLM evaluators, fostering ongoing research and
          development. We also raise concerns about potential biases in LLM
          evaluators, particularly towards LLM-generated content, and suggest
          including systems that integrate LLM evaluators in their design (e.g.,
          as re-rankers or for training data) to understand their influence and
          potential for ``gaming the metrics'' and adversarial moves.


\end{description}



==> opportunity-concerns.tex <==
\section{Opportunities and Concerns}
\ld{authors, please respond here.}


\ld{Assuming you don't agree with one of the extreme perspectives, what concerns do you have, that need to be studies or addressed before we wholeheartedly diver into an  LLM-without-humans evaluation?  }

\ld{Unbeknownst to us, what could go wrong with an LLM-evaluator?}



\newpage{}

\subsection{Dangers, Risks, and Concerns About Incorporating LLM Evaluators}

% \subsubsection{Fundamental Risks of LLM-Based Evaluation}

% The following issues arise when LLMs are used both as part of the system and the evaluator.

% \paragraph{Risk of Circular Evaluation}  
% If LLMs are both generating system outputs and evaluating them, the evaluation process risks becoming self-reinforcing rather than genuinely informative. This circularity undermines the credibility of the evaluation, as models may be optimized to align with the LLM’s biases rather than real-world relevance assessments (linked to 1.2 Synthetic Validation).

% \paragraph{LLM Is Just a Reranker (Charlie’s Thoughts)}  
% If the primary goal is traditional relevance ranking, and an LLM is accepted as an evaluator, then an LLM-based reranker (such as UMBRELA) effectively defines perfect ranking. If such a system is too expensive for direct deployment, then evaluating a cheaper model against UMBRELA may serve as a viable alternative.

% However, if UMBRELA is both the final-stage ranker and the evaluator, then evaluation risks becoming trivial---ranking is "solved" by definition under this closed system. This raises deeper philosophical concerns about what evaluation means in an LLM-dominated IR landscape.


% \paragraph{Hidden Contamination}
% As system developers and LLM evaluators often work independently, there is a risk that a system may unintentionally incorporate elements of the LLM evaluator’s methodology into its own design. This accidental circularity can lead to artificially high scores in automated evaluations, despite no actual improvement in system quality under human judgment.

\subsubsection{Fundamental Risks of LLM-Based Evaluation}

The following risks emerge when LLMs are used both as part of the system and as evaluators, creating potential feedback loops that distort evaluation outcomes.

\paragraph{Risk of Circular Evaluation}  
When LLMs serve as both content generators and evaluators, the evaluation process risks becoming self-reinforcing rather than genuinely informative \citep{alaofi2024generative, clarke2024llm,wei2024rethinking}. Models may be optimized to align with the LLM's biases rather than real-world relevance assessments, undermining the credibility of the evaluation (linked to 1.2 Synthetic Validation). This feedback loop creates an illusion of progress while failing to ensure that retrieval quality genuinely improves for human users.

\paragraph{Unintended Circularity Contamination}  
Even when system developers and LLM evaluators operate independently, unintentional contamination can occur. A system may unknowingly integrate elements of an LLM evaluator’s methodology, either through training data, algorithmic choices, or shared heuristics. This accidental feedback loop can lead to inflated performance in LLM-based evaluations without real improvements in retrieval quality under human assessment \citep{singh2024evaluation,sainz2023nlp,roberts2023data}.

\paragraph{LLM Is Just a Reranker (\Charlie{}’s Thoughts)}  
As demonstrated in Figure \ref{fig:charlie-rag24-plot}, if an LLM is accepted as an evaluator, then using an LLM-evaluation-based reranker\cite{ma2023finetuning,ma2023zeroshot}---such as {\sc umbrela}---effectively defines perfect ranking within its own system. If the LLM evaluator is too costly for deployment, it can still serve as a high-fidelity evaluation tool for comparing cheaper models. However, if the LLM evaluator is both the final-stage ranker and the evaluator, then evaluation risks becoming trivially circular---ranking is ``solved'' by definition within this closed system. This raises deeper philosophical concerns about whether LLM-based evaluation can still serve as a meaningful measure of real-world retrieval performance \citep{gao2024llmenhanced}.

\paragraph{Loss of Diversity in Evaluations}  
Relying exclusively on LLM-based judgments may homogenize responses, penalizing creative, diverse, or unconventional yet valid outputs \citep{padmakumar2023writing,bhatt2024extrinsic}. Human assessors often recognize subtle aspects of novelty and diversity that LLMs fail to capture, potentially leading to an overly narrow definition of relevance \citep{si2024evaluating}.

\paragraph{Overfitting to a Single Metric (\Nick{})}  
Optimizing systems to perform well on a single LLM-derived evaluation metric can lead to degradation on other important measures \citep{zhang2023constructing,zhang2020better,scheltema2024recommender}. Industry experience has shown that systems trained exclusively for high NDCG scores may deteriorate in user-centric metrics such as click-through rate, dwell time, and spam resistance.

\subsubsection{Concerns about the use of LLMs}

The following well-known issues with LLMs cast a shadow of a doubt on the validity of LLM evaluations.

\paragraph{Biases and Failures of LLM Evaluators}  
LLMs frequently overgeneralize, struggle with long-tail queries , and exhibit systematic biases\citep{salecha2024large,vanderweij2024ai,hauser2025large}---such as favoring verbose, authoritative-sounding responses or being overly sensitive to prompt phrasing . These biases can distort evaluations, favoring certain response styles over actual relevance.

% \paragraph{LLMs Make Systematic Mistakes (\Laura{}'s Stomach Aches)}  
% LLMs often fail in basic ways, raising concerns about their fundamental reliability as evaluators. These failures include:  
% \begin{itemize}
%     \item Injecting unrelated content into responses
%     \item Misinterpreting prompts or confusing instruction wording with the context
%     \item Providing incorrect answers
%     \item Failing to follow step-by-step logical reasoning
% \end{itemize}
Such issues suggest that LLM evaluators require significant oversight and correction mechanisms before they can be trusted for large-scale evaluations.

\paragraph{Content-Injection Attacks Against LLM-Judges}  
\ld{include references from above}
LLM-based evaluators are vulnerable to adversarial manipulation. Carefully crafted prompts or content injection techniques can steer LLMs toward biased or incorrect judgments. Additionally, positioning effects---where slight changes in ranking order lead to different evaluations---suggest that LLMs may lack evaluation stability.

\subsubsection{Issues with Future LLMs}

\paragraph{LLM Model Drift}  
LLMs are not static; their behavior evolves as they are updated \citep{chen2023chatgpt}. Future versions of an LLM may evaluate relevance differently than earlier ones, creating inconsistencies in longitudinal evaluations. This drift is particularly concerning if models are inadvertently trained on their own prior outputs.

\paragraph{Self-Training Biases}  
\ld{maybe merge with LLM model drift?}
The growing trend of training LLMs on LLM-generated data raises concerns about concept drift and quality degradation over time \citep{yeo2024selftraining}. If models increasingly rely on their own outputs as training data, they may reinforce existing biases, amplifying errors rather than correcting them \citep{gerstgrasser2024model,dohmatob2024demystified}.

 \paragraph{LLMs Are Trained on Test Collections}  
\ld{compress}
LLM-based evaluations may be inadvertently influenced by the training data, creating an illusion of high accuracy that does not generalize to real-world conditions (linked to 3.2 Synthetic Training). If test collections were part of an LLM’s training data, evaluations risk being artificially inflated due to test set memorization rather than genuine generalization \citep{zhou2023dont}.

A major concern is that many widely used IR test collections have likely been incorporated into LLM training datasets, leading to test data leakage. This contamination inflates evaluation scores, as the model may have memorized test examples rather than reasoning about relevance. Future IR test collections may face similar risks, necessitating strict controls on dataset provenance.

\subsubsection{Overfitting to LLM-Based Evaluation}

\paragraph{Overfitting to the LLM-Judge}  
Systems trained to maximize agreement with an LLM judge (3.2) risk developing artificial artifacts that perform well in evaluation but fail in real-world applications \citep{ailem2024examining,bordt2024elephants}. Such systems may exploit LLM-specific scoring heuristics rather than optimizing for genuine user satisfaction.

\paragraph{Evaluation to Outperform the SOTA}  
Standard evaluation methods, such as per-label agreement and leaderboard correlation, do not necessarily capture the most important use case: determining whether a novel system truly outperforms all state-of-the-art systems \citep{ioannidis2005most,lundberg2024origins}. 
We need a continuous study of new systems (based on novel paradigms) along with novel meta-evaluation strategies to test whether synthetic test collections support such conclusions.
%LLM-based evaluation pipelines must be stress-tested to ensure they do not simply validate incremental performance gains that are not meaningful in real-world scenarios.

\paragraph{Gaming LLM-Judge as a Ranker}
\ld{merge with Circularity}
Since many LLM's fail to detect mistakes made by LLMs \citep{meta2024selftaught}, a growing concern is that model developers may optimize their systems to exploit LLM-based evaluation heuristics rather than improving actual retrieval effectiveness. Since any LLM-based evaluator can be deployed as part of a ranking system, this feedback loop creates self-reinforcing evaluation artifacts that perform well under LLM-based relevance assessments but fail under manual judgments. 

A concrete example of this effect is presented in \citet{clarke2024llm}. In Figure \ref{fig:charlie-rag24-plot}, we demonstrate that this leads to a divergence in the leaderboards.


 
\subsection{Opportunities of LLM Evaluation}  


 \ld{Beyond the usual. Do you see particular opportunities that are often forgotten in this discussion?  (beyond cost, applicability for GenIR)}
 \oz{I think that the canva example is a good one, synthetic training data, personalization (infinite qrels) }


Beyond the well-known benefits of cost reduction and applicability to generative IR (GenIR), LLM-based evaluators introduce several underexplored opportunities that could substantially improve retrieval evaluation methodologies.

% \paragraph{Scalability}  
% LLM-based evaluators have the potential to dramatically scale evaluation efforts, surpassing the constraints of manual human assessments. This scalability enables researchers to evaluate larger datasets, cover a wider variety of retrieval tasks, and conduct evaluations more frequently (linked to 4.2 Human-LLM Coworking).  

% \paragraph{Speed and Ease of Availability (\Mark{})}  
% Beyond reducing the costs of manual judgment, one of the most transformative benefits of LLM-based evaluation is speed. Unlike human assessors, who require coordination, training, and extensive annotation time, LLMs can generate relevance labels almost instantly. This lowers the barrier to entry for retrieval evaluation, allowing researchers to explore multiple retrieval tasks and application domains that were previously constrained by time and resources.  

\paragraph{New Evaluation Paradigms}  
LLMs enable novel evaluation methodologies that go beyond traditional graded relevance judgments.
Techniques such as pairwise comparisons, claim-based scoring, and reasoning-chain evaluations introduce structured, nuanced assessments that complement traditional evaluation metrics.
By incorporating these richer methodologies, LLM-based evaluations can capture complex relevance relationships that may be difficult for human assessors to express explicitly.  

\paragraph{Whitebox Relevance Labels (\Laura{})}  
Unlike traditional human annotations, LLM-based evaluators can provide detailed justifications for relevance judgments, making the evaluation process more transparent and interpretable. Instead of just assigning a relevance score, LLMs can:  
\begin{itemize}  
    \item Highlight specific passages that contribute to relevance.  
    \item Align judgments with formal annotation guidelines.  
    \item Provide rationales and explanations, making it easier to understand why a document was deemed relevant.  
\end{itemize}  
While human judges could theoretically offer similar annotations, inter-annotator variability and inconsistencies often reduce the utility of these artifacts. LLMs, if properly calibrated, could generate structured and consistent rationales, improving the reliability of evaluation outputs.  

\paragraph{Hybrid Evaluation Setups}  
LLMs can function as assistants rather than replacements in the evaluation process, supporting hybrid evaluation setups where they help pre-screen, cluster, and organize assessments before final human verification. This approach improves efficiency by reducing the cognitive load on human assessors, enabling them to focus on more ambiguous or high-stakes judgments. Hybrid setups preserve the strengths of human evaluation while leveraging the scalability and speed of LLMs.  

\paragraph{Rationales for User Interaction Data and Relevance (\Charlie{})}  
One of the longstanding challenges in IR evaluation is interpreting implicit user signals, such as click patterns and search behavior. LLMs could serve as interpretive layers, translating observed user interactions into explicit explanations of information needs.  

For example, if a user skips a highly ranked result (A) but clicks on a lower-ranked result (B), an LLM could be prompted to explain the underlying intent behind this click inversion. This capability would allow researchers to generate hypotheses about user behavior, better align evaluation metrics with real-world user preferences, and gain deeper insights into why certain retrieval models perform well or poorly.


\paragraph{Adressing Human Priming and LLM In-Context Learning}  
Human evaluators exhibit priming effects, where their initial judgments subconsciously shape later assessments. This process helps assessors familiarize themselves with the task, refine their notion of relevance, and adapt dynamically to nuanced cases. Superficially, this resembles in-context learning in LLMs, where prompt examples influence generated responses. However, there are fundamental differences between these two processes.  

Unlike human assessors, who refine their judgments based on experience, expertise, and external knowledge, LLMs rely entirely on training data and statistical patterns. Human priming is an adaptive cognitive process, while LLM in-context learning is a fixed mechanism of pattern recognition. This distinction has significant implications for LLMs as evaluators:  

\begin{itemize}  
    \item Humans dynamically adjust their judgments, applying reasoning, background knowledge, and context—LLMs operate within fixed, pre-learned representations.  
    \item LLMs exhibit greater consistency but are prone to reinforcing biases and overfitting to prompt examples, whereas humans adapt their criteria based on evolving context.  
    \item LLMs process relevance differently, often favoring LLM-generated content over human-assessed relevance. This could distort evaluations, amplifying algorithmic biases and misaligning search systems with actual user needs.  
\end{itemize}  

While LLMs offer scalability and consistency, their lack of human-like adaptation raises concerns about reinforcing biases, overfitting to prompt designs, and misrepresenting human information needs in search evaluations. Understanding these differences is crucial in designing LLM-assisted evaluation pipelines that preserve human-level nuance while leveraging automation benefits.



\subsection{Concerns About Supporting Human Labeling With LLM Evaluator Output}

While LLMs can provide relevance label proposals to be verified by human assessors (linked to 4.1), their influence introduces risks related to bias reinforcement, over-reliance, and transparency. To ensure that LLM-human collaboration enhances rather than compromises evaluation quality, it is crucial to recognize these challenges and their implications.

\paragraph{Risk of Over-Reliance, Automation Bias, and Bias Reinforcement}  
Humans tend to perceive machine-generated outputs as authoritative, leading to blind acceptance of LLM-generated labels  (cf\. Section \ref{sec:llm-human-coworking}) \citep{distrust2023,fok2024search,krugel2021zombies}. This effect is particularly concerning when the model’s reasoning is opaque, making it difficult for annotators to challenge incorrect judgments.  Over time, reliance on LLM outputs may reinforce self-consistent but incorrect decision patterns, amplifying pre-existing model biases. This can result in a rubber-stamping effect, where human oversight becomes a superficial validation rather than a genuine evaluation.
 

% \paragraph{Automation Bias and the Authority Effect}  
% 

\paragraph{Transparency and Explainability in LLM-Assisted Judgment}  
A key concern is the lack of transparency in LLM-generated relevance labels. Unlike human assessors, who can justify, adapt, and refine their judgments, LLMs produce fixed, pre-trained assessments with limited interpretability. If assessors are presented with opaque model outputs without supporting explanations, they may struggle to critically assess LLM decisions, increasing the risk of uncritical acceptance rather than informed oversight. This raises broader concerns about how to balance human reasoning with LLM-generated judgments while maintaining evaluation integrity \citep{liao2023ai,ji2024detecting}.

\subsection{Concerns of Nugget-Based Evaluation}

This setup preserves human control over the definition of relevance, paradigms of LLM-assisted evaluation (linked to 4.2) can be used to divide the label of  (manually) defining relevant elements, then using LLMs for low-level text matching.

A core challenge is ensuring that the defined nugget set comprehensively captures relevance \citep{lin2006different,rajput2011nugget}. 

% If the set is too narrow, it may fail to identify valid relevant responses, unfairly penalizing some systems. Conversely, if it is too broad, it may lack discriminative power, failing to distinguish highly relevant content from merely related information.  

% A further concern is that relevance may not always be reducible to a predefined set of nuggets. Some system outputs may exhibit holistic qualities, such as coherence or informativeness, that do not align neatly with nugget-based evaluation. This raises questions about how well a nugget-centric approach can generalize across different retrieval tasks and domains.

\subsection{Missing Key Information in Evaluation (\Faegheh{})}  
Systematic discrepancies may emerge when relevance is decomposed into explicit criteria.
This is because of the presence of latent, unaccounted-for factors that influence human judgment may are not be explicitly modeled.

% If evaluation is broken into distinct dimensions (e.g., factual accuracy, specificity, coherence), and even if humans and LLMs agree perfectly on each of these dimensions, differences in overall assessments may persist. 
This suggests that both LLMs and human judges may rely on implicit factors that shape their final judgments, leading to fundamental misalignment even when explicit evaluation criteria match \citep{uprety2018modeling,liu2024hdeval}.


==> scope.tex <==

\section{Categorizing Evaluation Scenarios}
\label{sec:scenarios}

The development of new LLM-based evaluators and LLM-based IR systems results in a range of possible configurations. Some of these are valid, while others may be invalid due to issues such as circularity or overfitting. 
% Evaluating LLM-based IR systems with LLM-based evaluators presents challenges related to validity, circular evaluation, and metric overfitting.
To mitigate these concerns, we define four key dimensions that shape the evaluation process.


\paragraph{Dimension 1: Validation Approach}

How is an evaluator/system validated---against human data or LLM metrics?

\begin{description}
    \item [1.1 Validated Against Humans:] The traditional approach for validating any system or evaluator involves using human data, such as relevance labels, search logs, panel studies, or lab experiments. For example, a SIGIR paper might compare human-judged NDCG scores with results from human-conducted lab studies.

    \item [1.2 Validated Against (Multiple) LLM Evaluators:] To complement human data, new evaluators or systems can be assessed against LLM-based evaluators. Using multiple evaluation methods helps prevent overfitting to a single metric---especially when that metric is derived from an LLM rather than human judgment.
\end{description}

\paragraph{Dimension 2: Evaluation Purpose}

Is the goal to develop an evaluator or a deployable system?

\begin{description}
    \item [2.1 LLM Evaluation Metric:] This approach focuses on developing LLM-based evaluation methodologies, such as relevance labeling, nuggetization, claim-based scoring, and pairwise ranking. These methods must be rigorously validated against human data (1.1) before they can be trusted. Papers that identify or mitigate flaws in evaluation methods are highly valued at SIGIR. While validating against other LLM evaluators (1.2) is less reliable, cross-checking can still offer useful insights.

    \item [2.2 Deployable System:] When designing a deployable system that utilizes an LLM evaluator, validation should be conducted against human data (1.1) to address circularity concerns. Conversely, if the system does not rely on LLMs---such as in low-latency applications---evaluation against LLM-based metrics (1.2) becomes permissible. Regardless of the approach, the goal should be to demonstrate improvements across multiple evaluation methods to avoid overfitting to any single LLM-based metric.
\end{description}

\begin{table}[tb]
\caption{Differences between IR Systems and LLM Evaluators.
\label{tab:dim12}
}
\begin{footnotesize}
\begin{tabular}{ccc}
\toprule 
Dim 2 / Dim 1 & Validate  & Validate against \tabularnewline
 & against people & multiple metrics\tabularnewline
\midrule 
LLM Evaluator & Evaluation paper & Increased Trust\tabularnewline
Deployable System & Traditional (e.g. Cranfield) & Retrieval/RAG/etc paper\tabularnewline
% Dim 2 / Dim 1 & Validate  & Validate against \tabularnewline
%  & against people & multiple metrics\tabularnewline
% \midrule 
% Synthetic Metric & A: New! & B: not important\tabularnewline
% Deployable System & C: Cranfield, A/B \& co & D: attempt to curb issues\tabularnewline
\bottomrule 
\end{tabular}
\end{footnotesize}
\end{table}

\paragraph{Dimension 3: Evaluator-System circularity}

%What data sources does the system rely on?
To which extent is the IR system using code or training data from the LLM evaluator?

\begin{description}
   \item [3.1 System runs the LLM evaluator at query time:]  
    In this scenario, the system directly incorporates the LLM evaluator during retrieval. For example, it may generate LLM-based relevance labels for the top-\textit{k} results and use these labels to rerank documents before presenting them to the user. Another example includes using an LLM-based hallucination-checking metric to filter RAG-generated responses prior to display. In such cases, human evaluation (1.1) is essential, as LLM evaluators would likely overestimate the system’s quality due to circularity concerns.


\item [3.2 System trained on LLM evaluator data:]  
    When the system is trained on LLM-generated labels instead of human-provided ones -- such as a ranker fine-tuned on LLM-generated relevance scores -- human evaluation (1.1) becomes necessary to prevent circularity and inflated performance assessments.

\item [3.3 Independently developed system:]  
    This category includes traditional IR systems that neither rely on synthetic training data nor employ LLM-based evaluation processes for reranking. Such systems can  be evaluated using LLM-based evaluators (as demonstrated in the literature \citep{thomas2024large}). Confidence in these evaluations increases when a diverse suite of independent LLM evaluators yields varied metrics (1.2). As research continues to uncover the flaws, correlations, and properties of LLM evaluators, the potential for fair and informative evaluations will improve.

\end{description}

\paragraph{Dimension 4: Human Involvement}

How much human oversight is present in the evaluation process?

\begin{description}
     \item [4.1 LLM-Judge:]  
    Fully automatic evaluation where LLMs generate labels without any human oversight or verification. While efficient, this approach risks reinforcing LLM-specific biases and systemic errors.


    \item [4.2 LLM Labels with Human Verification:]  
    LLMs generate initial labels, which are then verified and corrected by human assessors. The key challenge lies in developing processes that lead to genuine human verification as opposed to over-reliance  and blind trust \cite{fok2024search} in the LLM.

    \item [4.3 Human Judge with Low-Level LLM Support:]  
    Humans lead the evaluation process, with LLMs offering auxiliary support (e.g., suggesting lexically similar passages or pre-screening harmful content). While this approach can enhance efficiency, it bears a small risk to subtle biases that could influence outcomes.

    \item [4.4 Fully Manual Judgments:]  
    Evaluation relies entirely on human-annotated test collections (e.g., TREC), avoiding synthetic biases but requiring significant time and resources to obtain high-quality relevance labels.

\end{description}

\section{LLM evaluation: Concerns and Considerations}
A core challenge in LLM-based IR evaluation is avoiding circular validation (3.1/2.1), where a system is both built using and evaluated by the same LLM-based evaluation approach. This issue becomes especially problematic if the LLM methodology has not been rigorously validated against human data (1.1). The risk is most pronounced in systems that include LLM-Judge Reranking (3.1) or are trained on synthetic data (3.2), where the evaluation pipeline relies on outputs from a similar LLMs as used in the evaluation. While LLM Labels with Human Verification (4.2) can mitigate this risk, the verification process must be substantial enough to ensure genuine quality control rather than a superficial approval step.


To ensure evaluation validity, deployable systems (2.2) should be tested against multiple validated metrics (1.2) instead of overfitting to a single measure. This principle is already standard practice in industry: for example, ranking teams routinely balance NDCG, click-through rate, dwell time, and spam resistance to prevent overfitting to any single metric. However, a lingering concern is whether offline metrics are diverse enough to provide a similar guardrail.


Given their computational cost, synthetic evaluation methodologies (2.1) -- including nuggetization and pairwise preference labeling -- are better suited as high-quality validation tools rather than components of a deployed system. However, should an LLM evaluation process be integrated into the IR system, the experimental setup is prone to validity concerns \cite{clarke2024llm}.

With sufficient validation and appropriate guardrails, synthetic evaluation methods can be incorporated into hybrid evaluation setups (4.3), where humans retain primary oversight while leveraging LLM assistance to improve efficiency. Nonetheless, fully manual judgments (4.4) remain the gold standard for ensuring evaluation integrity. Evaluation venues such as TREC or NTCIR could play a role in coordinating an ongoing collaborative test collection building effort, where teams contribute both systems and evaluators which are both evaluated with human assessments.


LLM-based systems are not exempt from conventional risks associated with machine learning development practices. Data leakage between training and testing datasets can lead to inflated estimates of real-world performance. Similarly, over-fitting to limited training data has the same consequences. There may be new situations where these risks are further obfuscated by being masked within an intermediary LLM used as part of the train-test-validate system setup.  Contemporary LLM-Eval practices, particularly those involving synthetic training data (3.2), carry the potential for data leakage and overfitting. However, the use of synthetic data does not automatically invalidate an evaluation. Instead, we advocate for a careful examination of potential implications, complemented by the implementation of guardrails and additional diagnostic tests to monitor for unintended effects.

These potential issues underscore the importance of trusted, human-annotated benchmarks (3.3, 4.4) as essential foundations for evaluating new methods. Human-generated labels remain the most reliable safeguard against unintended artifacts, ensuring evaluations reflect genuine improvements rather than exploiting systemic biases.


\section{Adversarial Risks}

\ld{This section is somewhat lost here. Not sure where it would best fit into the story.  Should it be its own trope? Thoughts?}

While our primary concern is evaluation in good-faith settings, we cannot ignore the risks posed by adversarial actors. 
As LLMs become more integrated into ranking and evaluation,
they may unintentionally favor LLM-generated content or be manipulated through search engine optimization (SEO) techniques.
\citet{kurland2022} conceptualize the Web as a competitive search environment,
where document authors actively optimize content to improve their ranking.
Game-theoretic analysis shows that the probability ranking principle 
(PRP) is suboptimal in such settings, as it tends to reinforce dominant topical content at the expense of diversity~\cite{basat2015}.
\citet{bardas2025} recently showed that LLMs can be used to modify document content to boost 
rankings under two rankers: the feature-based Learning-to-Rank approach LambdaMART and the dense retrieval 
method E5~\cite{wang2024}. LLM-powered SEO tools are likely 
already employed, aiding content creators in ``white hat'' SEO. However, adversarial actors using
``black hat'' SEO, can apply similar techniques to distort search rankings, spread misinformation, or amplify propaganda.

The increasing reliance on LLMs for both ranking and evaluation compounds these concerns.
If LLMs systematically favor synthetic content
-- especially when adversarial content is introduced -- it increases the risk of reinforcing biases introduced earlier in the retrieval pipeline.
This feedback loop would likely incentivize content creators to generate synthetic content for SEO purposes, further amplifying its dominance over human-authored documents.
Consequently, evaluation outcomes may become skewed, retrieval effectiveness obscured, and ranking metrics less reliable.
Although adversarial manipulation is not the primary focus of this work,
the integrity of evaluation methods must remain a central consideration.
A system that fails under standard conditions is unlikely to be resilient against adversarial interference.
Future research should explore mechanisms for identifying and mitigating such risks,
ensuring that \emph{any} evaluation frameworks remain robust even in competitive and adversarial retrieval environments.

% Commenting out for final editing
% \paragraph{`Spam SEO' / Bad Actor \ld{out of scope?} \pb{none of this feels at all new in the context of web search over the last 2.5 decades, barring it's an LLM rather than a human directly consuming the ranking outputs}}
% A key incentive for maintaining web content is information warfare, where actors attempt to manipulate information for strategic gain.

% Consider the case of spammers, where an actor has an agenda and aims to manipulate system outputs by exploiting SEO vulnerabilities rather than following ethical guidelines. Although the spammer does not control the LLM itself, they can influence the web content that is crawled, stored in a search index, and later retrieved in a Retrieval-Augmented Generation (RAG) system. By strategically generating synthetic content, they can shape the context that an LLM uses, thereby influencing the generative process.

% From this perspective, the ranking step of a RAG system becomes less critical than the ability to control the generated outputs. A key concern is whether bad actors can systematically steer the model’s responses by manipulating indexed content.

% Looking ahead, we expect rapid adoption of reinforcement learning in retrieval systems. This introduces new risks, particularly when adversarial actors interact dynamically with one another. A crucial question is how the incentive structure of bad actors evolves as these systems become more sophisticated. While direct control over the LLM remains unlikely, adversaries may still craft and maintain web content specifically designed to affect the model’s generative process.




% In the remainder of this paper, we explore these concerns in detail, present empirical studies illustrating their effects, and outline best practices for deploying guardrails to mitigate identified risks.




\begin{table*}
\caption{Combinations of different evaluator approaches (Dimension 3) with different forms of ground truth labels (Dimension 4) are prone to different LLM-evaluation scenarios. \label{tab:dim34}}
\begin{tabular}{l|l l l }
\toprule
 & 3.1 System includes & 3.2 Training on  & 3.3 Traditional IR System \tabularnewline
 & LLM-judge Reranker & Synthetic Data & \tabularnewline
\midrule
4.1 LLM-judge & \textbf{Circularity} &  \textbf{Circularity} & Confirmed by Meta-Evaluations\tabularnewline
4.2 LLM Labels with Human Verification &  Check: ``Blind trust of humans?''&  Check: Data Leakage  & Confirmed by Meta-Evaluations\tabularnewline
%\hline 
4.3 Human with Low-Level LLM support & Check: ``Are Humans necessary?'' & Check: ``Turing test'' & Assessment Interface\tabularnewline
%\hline 
4.4 Fully Manual Judgments & Baseline for checking Circularity & Check: Synthetic Testcollections & \textbf{Tried and True}\tabularnewline

%\hline 
\bottomrule 
\end{tabular}

\end{table*}



==> short-opinions.tex <==

\begin{description}
    \item[Very optimistic perspective:]  Empirical studies demonstrate that it is safe to replace human judges with LLM-simulations. % \ld{I hope nobody falls in this camp}
    \item[\Charlie{}'s perspective:] We can fire all but the most careful and fully trained human assessors.  We can trust LLM evaluations, as long as we avoid issues of circularity and adversarial attacks.
    \item[\Faegheh{}'s perspective:] LLM-evaluations are essential to develop future conversational IR systems. Once we land on a local optima,
human evaluation can find the problems, and the models can
be further developed and optimized.
    \item[\Peter{}'s perspective:] Human assessors are finite and insufficiently variable; appropriately modeled LLM-simulations can scale up variability to better reflect true user populations.
    \item[\Ellese{}'s perspective:] 
    LLM-simulations can be reliably used in place of human judges, but with some human oversight to ensure their accuracy.
    \item[\Mark{}'s perspective] I think what we're finding with LLMs is that we can mostly replace those workers with an automated labeling approach. However, those labels need to be validated against high quality human relevance assessments.    \item[\Nick{}'s perspective:] Careful study of real people can validate expensive LLM metrics/models, which in turn can sometimes be used to evaluate an actual IR (retrieval, rag, conversation, etc) system.
    \item[\Oleg{}'s perspective] LLMs undeniably advance IR, but must be adopted cautiously. They simulate past trends and cannot fully capture human variability or anticipate new user behaviors.
    \item[\Laura{}'s perspective:] LLM-simulations can fix judgment holes or perform syntactic tasks like align nuggets, match gold answers, or clean up documents, but nothing else. % Nick comment: Wasn't there a paper that said this causes a bias, to use a mix of labels from two different labeling systems (mixing human and llm is bad, but also probably bad to mix e.g. nist and turkers, etc)
    % \item[\Jeff{}'s] perspective] \ld{here}
    \item[Extremely cautious perspective:] LLM-simulations cannot be used as any valid form of evaluation.
\end{description}

==> trope-figure.tex <==


### **Figure: Interaction of LLM-Eval Tropes and Their Effects**
Below is a conceptual figure depicting how the identified LLM-Eval tropes interact with each other and influence the evaluation process, IR system development, and human oversight.

```mermaid
graph TD
    subgraph Invalid_Evaluation[Invalid Evaluation Tropes]
        A[Circularity] --> B[LLM Narcissism]
        B --> C[LLM-Eval as Ranker]
        C --> D[Test Set Leak Inflation]
    end

    subgraph Misled_Systems[Misled System Tropes]
        E[Synthetic Overfitting] --> F[Wrong Data Usage]
        F --> G[Self-Training Collapse]
    end

    subgraph Misled_Humans[Misled Human Evaluator Tropes]
        H[Loss of Evaluation Diversity] --> I[Rubber-Stamp Effect]
        I --> J[Overreliance & Automation Bias]
    end

    %% Cross-connections
    A --> E
    D --> G
    F --> H
    B --> H
    I --> G
    C --> E

    %% Human guardrails
    subgraph Guardrails[Guardrails & Mitigations]
        K[Multiple Metrics & Diverse Evaluations]
        L[Vigilance Tests & Human Verification]
        M[Stepwise Reasoning Chains]
        N[Privileged Information Protection]
    end

    %% Connecting guardrails to tropes
    K --> A
    K --> E
    L --> I
    L --> J
    M --> C
    M --> D
    N --> D
    N --> F
```

---

### **Explanation of the Figure:**
- **Invalid Evaluation Tropes:** Issues like *Circularity*, *LLM Narcissism*, and *Test Set Leak Inflation* form a chain where flawed evaluation processes can propagate errors into IR system performance.
- **Misled System Tropes:** Overfitting to synthetic data (*Synthetic Overfitting*) and dependence on *Wrong Data Usage* can culminate in *Self-Training Collapse*.
- **Misled Human Evaluator Tropes:** Human-centric issues like the *Rubber-Stamp Effect* and *Overreliance & Automation Bias* lead to *Loss of Evaluation Diversity*.
- **Cross-Connections:** Many tropes influence each other. For example, *LLM Narcissism* contributes to both system overfitting and reduced evaluation diversity.
- **Guardrails & Mitigations:** Strategies like *Multiple Metrics*, *Human Verification*, and *Privileged Information Protection* mitigate the risks posed by these tropes.

